BosonSampling.jl: A Julia package for quantum multi-photon interferometry

We present a free open source package for high performance simulation and numerical investigation of boson samplers and, more generally, multi-photon interferometry. Our package is written in Julia, allowing C-like performance with easy notations and fast, high-level coding. Underlying building blocks can easily be modified without complicated low-level language modifications. We present a great variety of routines for tasks related to boson sampling, such as statistical tools, optimization methods, classical samplers and validation tools.

==> code-samples/dark_counts.tex <==
\begin{Shaded}
\begin{Highlighting}[]
\CommentTok{\# define a new measurement type of a simple dark}
\CommentTok{\# counting detector}

\KeywordTok{mutable struct}\NormalTok{ DarkCountFockSample}
    \OperatorTok{\textless{}:}\DataTypeTok{ OutputMeasurementType}
    \CommentTok{\# observed output, possibly undefined}
\NormalTok{    s}\OperatorTok{::}\DataTypeTok{Union\{ModeOccupation, Nothing\}}
    \CommentTok{\# probability of a dark count in each mode}
\NormalTok{    p}\OperatorTok{::}\DataTypeTok{Real}
    \CommentTok{\# instantiate if no known output}
    \ControlFlowTok{if}\NormalTok{ (}\FunctionTok{DarkCountFockSample}\NormalTok{(p}\OperatorTok{::}\DataTypeTok{Real}\NormalTok{) }\OperatorTok{=}
    \FunctionTok{isa\_probability}\NormalTok{(p))}
        \FunctionTok{new}\NormalTok{(}\ConstantTok{nothing}\NormalTok{, p)}
    \ControlFlowTok{else}
         \FunctionTok{error}\NormalTok{(}\StringTok{"invalid probability"}\NormalTok{)}
\ControlFlowTok{end}

\CommentTok{\# works DarkCountFockSample(0.01)}
\CommentTok{\# fails DarkCountFockSample({-}1)}
\CommentTok{\# define the sampling algorithm:}
\CommentTok{\# the function sample! is modified}
\CommentTok{\# to take into account the new}
\CommentTok{\# measurement type this allows to}
\CommentTok{\# keep the same syntax and in fact}
\CommentTok{\# reuse any function that would have}
\CommentTok{\# previously used sample! at no cost}
\KeywordTok{function} \FunctionTok{sample!}\NormalTok{(ev}\OperatorTok{::}\DataTypeTok{Event\{TIn,TOut\}}\NormalTok{)}
    \KeywordTok{where}\NormalTok{ \{TIn}\OperatorTok{\textless{}:}\DataTypeTok{InputType}\NormalTok{,}
\NormalTok{           TOut }\OperatorTok{\textless{}:}\DataTypeTok{ DarkCountFockSample}\NormalTok{\}}

    \CommentTok{\# sample without dark counts}
\NormalTok{    ev\_no\_dark }\OperatorTok{=} \FunctionTok{Event}\NormalTok{(ev.input\_state,}
                       \FunctionTok{FockSample}\NormalTok{(),}
\NormalTok{                       ev.interferometer)}
    \FunctionTok{sample!}\NormalTok{(ev\_no\_dark)}
\NormalTok{    sample\_no\_dark }\OperatorTok{=}
\NormalTok{    ev\_no\_dark.output\_measurement.s}

    \CommentTok{\# now, apply the dark counts to}
    \CommentTok{\# "perfect" samples 1 with}
    \CommentTok{\# probability p, 0 with probability 1{-}p}
    \FunctionTok{observe\_dark\_count}\NormalTok{(p) }\OperatorTok{=}
    \FunctionTok{Int}\NormalTok{(}\FunctionTok{do\_with\_probability}\NormalTok{(p))}
\NormalTok{    dark\_counts }\OperatorTok{=}
\NormalTok{    [}\FunctionTok{observe\_dark\_count}\NormalTok{(ev.output\_measurement.p)}
\NormalTok{    for i }\KeywordTok{in} \FloatTok{1}\OperatorTok{:}\NormalTok{ ev.input\_state.m]}

\NormalTok{    ev.output\_measurement.s }\OperatorTok{=}
\NormalTok{    sample\_no\_dark }\OperatorTok{+}\NormalTok{ dark\_counts}
\KeywordTok{end}

\CommentTok{\#\#\# example \#\#\#}

\CommentTok{\# experiment parameters}
\NormalTok{n }\OperatorTok{=} \FloatTok{10}
\NormalTok{m }\OperatorTok{=} \FloatTok{10}
\NormalTok{p\_dark }\OperatorTok{=} \FloatTok{0.1}
\NormalTok{input\_state }\OperatorTok{=} \FunctionTok{first\_modes}\NormalTok{(n,m)}
\NormalTok{interf }\OperatorTok{=} \FunctionTok{RandHaar}\NormalTok{(m)}
\NormalTok{i }\OperatorTok{=} \FunctionTok{Input}\DataTypeTok{\{Bosonic\}}\NormalTok{(input\_state)}
\NormalTok{o }\OperatorTok{=} \FunctionTok{DarkCountFockSample}\NormalTok{(p\_dark)}
\NormalTok{ev }\OperatorTok{=} \FunctionTok{Event}\NormalTok{(i,o,interf)}

\FunctionTok{sample!}\NormalTok{(ev)}
\CommentTok{\# output:}
\CommentTok{\# state = [3, 1, 0, 3, 0, 1, 2, 0, 0, 0]}
\end{Highlighting}
\end{Shaded}


==> code-samples/event_HOM.tex <==
\begin{Shaded}
\begin{Highlighting}[]
\CommentTok{\# Define the input with one particle in}
\CommentTok{\# each input mode}
\NormalTok{r\_i }\OperatorTok{=} \FunctionTok{ModeOccupation}\NormalTok{([}\FloatTok{1}\NormalTok{,}\FloatTok{1}\NormalTok{])}
\NormalTok{i }\OperatorTok{=} \FunctionTok{Input}\DataTypeTok{\{Bosonic\}}\NormalTok{(r\_i)}

\CommentTok{\# Define the unbalanced interferometer}
\NormalTok{B }\OperatorTok{=} \FunctionTok{BeamSplitter}\NormalTok{(}\FloatTok{1}\OperatorTok{/}\FunctionTok{sqrt}\NormalTok{(}\FloatTok{2}\NormalTok{))}

\CommentTok{\# Define the output}
\NormalTok{r\_f }\OperatorTok{=} \FunctionTok{ModeOccupation}\NormalTok{([}\FloatTok{1}\NormalTok{,}\FloatTok{1}\NormalTok{])}
\NormalTok{o }\OperatorTok{=} \FunctionTok{FockDetection}\NormalTok{(r\_f)}

\CommentTok{\# Create the event}
\NormalTok{ev }\OperatorTok{=} \FunctionTok{Event}\NormalTok{(i,o,B)}
\CommentTok{\# Compute its probability to occur}
\FunctionTok{compute\_probability!}\NormalTok{(ev)}
\end{Highlighting}
\end{Shaded}


==> code-samples/partition_HOM.tex <==
\begin{Shaded}
\begin{Highlighting}[]
\NormalTok{i }\OperatorTok{=} \FunctionTok{Input}\DataTypeTok{\{Bosonic\}}\NormalTok{(}\FunctionTok{first\_modes}\NormalTok{(}\FloatTok{2}\NormalTok{,}\FloatTok{2}\NormalTok{))}

\NormalTok{set1 }\OperatorTok{=} \FunctionTok{Subset}\NormalTok{([}\FloatTok{1}\NormalTok{,}\FloatTok{0}\NormalTok{])}
\NormalTok{set2 }\OperatorTok{=} \FunctionTok{Subset}\NormalTok{([}\FloatTok{0}\NormalTok{,}\FloatTok{1}\NormalTok{])}
\NormalTok{interf }\OperatorTok{=} \FunctionTok{Fourier}\NormalTok{(}\FloatTok{2}\NormalTok{)}
\NormalTok{part }\OperatorTok{=} \FunctionTok{Partition}\NormalTok{([set1,set2])}

\NormalTok{(idx,pdf) }\OperatorTok{=}
\FunctionTok{compute\_probabilities\_partition}\NormalTok{(interf,part,i)}
\end{Highlighting}
\end{Shaded}


==> code-samples/thermalization.tex <==
\begin{Shaded}
\begin{Highlighting}[]
\ImportTok{using} \BuiltInTok{BosonSampling}
\ImportTok{using} \BuiltInTok{Plots; }\FunctionTok{pyplot}\NormalTok{()}

\NormalTok{n }\OperatorTok{=} \FloatTok{20}
\NormalTok{trunc }\OperatorTok{=} \FloatTok{10}
\NormalTok{T }\OperatorTok{=}\NormalTok{ OneParameterInterpolation}
\ControlFlowTok{for}\NormalTok{ x }\KeywordTok{in} \FloatTok{0}\OperatorTok{:}\FloatTok{0.01}\OperatorTok{:}\FloatTok{1}
\NormalTok{    i }\OperatorTok{=}
    \FunctionTok{Input}\DataTypeTok{\{T\}}\NormalTok{(}\FunctionTok{first\_modes}\NormalTok{(n,n),x)}
\NormalTok{    set1 }\OperatorTok{=}\NormalTok{ [}\FloatTok{0}\NormalTok{ for i }\KeywordTok{in} \FloatTok{1}\OperatorTok{:}\NormalTok{n]}
\NormalTok{    set1[}\FloatTok{1}\NormalTok{] }\OperatorTok{=} \FloatTok{1}
\NormalTok{    part }\OperatorTok{=} \FunctionTok{Partition}\NormalTok{([}\FunctionTok{Subset}\NormalTok{(set1)])}
\NormalTok{    F }\OperatorTok{=} \FunctionTok{Fourier}\NormalTok{(n)}
\NormalTok{    (idx,pdf) }\OperatorTok{=}
    \FunctionTok{compute\_probabilities\_partition}\NormalTok{(F,part,i)}
\ControlFlowTok{end}
\end{Highlighting}
\end{Shaded}

